Embodiment-Agnostic Action Planning via Object-Part Scene Flow

Observing that the key for robotic action planning is to understand the target-object motion when its associated part is manipulated by the end effector, we propose to generate the 3D object-part scene flow and extract its transformations to solve the action trajectories for diverse embodiments. The advantage of our approach is that it derives the robot action explicitly from object motion prediction, yielding a more robust policy by understanding the object motions. Also, beyond policies trained on embodiment-centric data, our method is embodiment-agnostic, generalizable across diverse embodiments, and being able to learn from human demonstrations. Our method comprises three components: an object-part predictor to locate the part for the end effector to manipulate, an RGBD video generator to predict future RGBD videos, and a trajectory planner to extract embodiment-agnostic transformation sequences and solve the trajectory for diverse embodiments. Trained on videos even without trajectory data, our method still outperforms existing works significantly by 27.7% and 26.2% on the prevailing virtual environments MetaWorld and Franka-Kitchen, respectively. Furthermore, we conducted real-world experiments, showing that our policy, trained only with human demonstration, can be deployed to various embodiments.

==> introduction.tex <==
\section{INTRODUCTION}
\label{sec:intro}
%
In Automatic Storehouse~(auto-store), Stock Keeping Unit (SKU) refers to a unique identifier of each product in the inventory management.
%
To enable the robotic system to handle a large variety of SKUs, we need instance segmentation, a fundamental vision task, to segment each SKU in the camera view. 
%,  is a fundamental vision task for sequential grasping. 
%
%For a large-scale picking pipeline that contains billions of SKUs, instance segmentation is a fundamental vision task for sequential grasping. 
%
%Especially, cluttered scenes are common.
By then, the instance-level masks can enable the robot arm to effectively pick the SKUs one by one.

%
Recent deep-learning approaches show promising performance for general Instance Segmentation (IS, Fig.~\ref{fig: teaser} top-left)~\cite{he2017mask,liu2018path,chen2018masklab}.
%
Yet, it remains challenging to tackle Unseen Object Instance Segmentation~(UOIS, Fig.~\ref{fig: teaser} top-middle), i.e., testing SKUs different from training SKUs.
%
While some recent works on UOIS~\cite{xie2020best,back2021unseen,xie2021unseen,zhang2022unseen} start to address the seen-unseen domain gap, they may not work well for large-scale storehouses with a huge amount and variety of SKUs.
%with distinctive appearances.

To improve the segmentation accuracy on unseen SKUs, the Self-Ensembling Instance Segmentation approach~(SEIS, Fig.~\ref{fig: teaser} top-right)~\cite{gu2021class,yang2022sesr} is proposed.
By acquiring quite a number of images prepared for each unseen SKU, teacher-student pseudo labeling can be exploited to enable the pre-trained model to fit the unseen objects.
%within.
Though human annotations are not required, the segmentation performance is still not satisfactory for successful grasping in practice, especially for crowded and chaotic scenes.
%
%Hence, the existing solutions cannot effectively handle the challenging large-scale Auto-Store environment.
Besides, existing solutions have two other issues for handling the challenging large-scale auto-store environment.
%
First, they heavily rely on manual efforts to tediously prepare a large volume of data 
%with annotated pixel-level masks 
for every single SKU.
%cost tedious human labor.
Second, for every new incoming SKU, the model has to be fine-tuned; doing so unavoidably
% \phil{for every single incoming SKU, we have to...} we have to repeatedly fine-tune the model as soon as new SKUs come
lower the practicality, efficiency, and scalability.

%
To meet these challenges, we develop~\ourmethod, a new patch-guided instance segmentation (Fig.~\ref{fig: teaser} bottom) solution for auto-store.
% To address the above problems, we modify \phil{don't say modify... which sounds small improvement over previous works} the task to Patch-Guided Instance Segmentation (\ourmethod, Fig.~\ref{fig: teaser} bottom). 
%
Without requiring
%No need of any 
scene-level data collection and tedious human annotations, we employ only a \textit{few image patches} prepared for each new SKU for predicting the object masks.
%to produce reliable mask results.
%
Compared with IS,~\ourmethod\ can well generalize to efficiently handle a large variety of unseen SKUs with much lower data-collection requirements.
%
Comparing with UOIS,~\ourmethod\ harnesses the strength of instance patches and is able to produce convincing masks accurately for auto-store picking. Further, using a well-trained~\ourmethod\ network for a known SKU database, we can directly deploy it to the robot system for real-time usage, without requiring any re-training and parameter tuning as in SEIS.

\begin{figure}[t]
	\centering
 \includegraphics[width=1.0\linewidth]{figs/Teaser.png}
 
	\vspace*{-3mm}
	\caption{Results on unseen SKUs produced by (i) the general Instance Segmentation (IS) method Mask R-CNN~\cite{he2017mask}, (ii) the Unseen Object Instance Segmentation (UOIS) method UOIS-2D~\cite{xie2021unseen}, (iii) the Self-Ensembling (SEIS) method SESR~\cite{yang2022sesr}, and 
 (iv)~\ourmethod~(ours). Clearly,~\ourmethod\ can generate more precise masks by leveraging only a few easily-obtainable SKU patches. 
 ``w/ sup'' and ``w/o sup'' mean with and without supervision.
	}
	\vspace*{-6mm}
	\label{fig: teaser}
\end{figure} 

As shown in Fig.~\ref{fig: teaser}, the SKU patch provides informative color and texture information of the target object instance. 
Intuitively, these features are strong prior knowledge that can guide the segmentor to achieve annotation-free and precise predictions on the unseen SKUs.
Importantly, SKU patches can be collected with very little effort without requiring any image annotation: it takes only a few seconds to capture 10 patches for an SKU with an industrial collection system~\cite{wei2019rpc,liu2020keypose}. 
% \\
% %
% Technically, each SKU patch provides RGB information of a single object instance under a specific pose. Given each new (unseen) SKU, its multi-view patches can be collected with very little effort. With an industrial collection system~\cite{wei2019rpc,liu2020keypose}, it takes only a few seconds to capture 10 patches for an SKU, without requiring any image annotation. 
% %take only 3s, which is much easier than image annotation.
% %
% The set of patches is a critical SKU reference.
% %
% with each patch represents an unique appearance of the associated object.
% \phil{don't say this... which may lead to questions on how to maximize the results by estimating the best view set... which is a very hard traditional CV problem}
% %
% Intuitively, they provide prior knowledge to guide the segmentor to achieve annotation-free and precise predictions on the unseen SKUs. 
% 
% For our proposed \ourmethod solution, 
So, the challenges lie in how to extract vision contexts from the SKU patches and use the patch-level information to guide the image-level instance segmentation.
%
Technical-wise, we propose a patch-guided transformer framework designed for SKU patches.
%
Our network consists of a patch-image correlation encoder, a patch-aware image decoder, and task heads. The encoder learns multi-level patch-image correlation through the cross-attention mechanism and outputs the calibrated image feature pyramid. The decoder aggregates the image features and learns a fixed number of compact instance embeddings. Then, the classification, box, and mask heads make predictions for each embedding. 
%Noted that the heavy computation cost in vision transformer~\cite{dosovitskiy2020image} is not applicable for a robot system, our network therefore is built upon an efficient transformer detector architecture~\cite{song2021vidt}. 

%
Extensive experiments show that \ourmethod\ is an effective solution for auto-store.
It can robustly provide instance masks for unseen SKUs, using only a few image patches.
Also, our Transformer~\ourmethod\ network achieves top precision and recalls on four benchmarks, outperforming
the state-of-the-art approaches. 
To test its practical performance, we deploy it on a real robot arm and use it to grasp unseen commodities in the storehouse.
SKU-Patch has a success rate of nearly 100\% on a wide variety of objects with different appearances.

%
Our contributions can be summarized as follows:
\begin{itemize}
    \item We formulate~\ourmethod, a new solution for segmenting mass unseen SKUs in auto-store, requiring only a few image patches and relieving us from tedious pixel-level annotations and incessant network tuning.
    \item We design the novel transformer-based~\ourmethod\ network to correlate local instance patches and global cluttered scenes, so as to fully exploit the patch information for accurate mask predictions of unseen objects.
    \item Extensive experiments on four benchmark datasets  show the top performance of~\ourmethod, compared with recent SOTA methods.
    Robotic bin picking demos on more than 50 different unseen SKUs further demonstrate the strong capability of~\ourmethod.
\end{itemize}




